Exploiting Student Parallelism for Efficient GPU Inference of BERT-like Models in Online Services

Due to high accuracy, BERT-like models have been widely adopted by text mining and web searching. However, large BERT-like models suffer from inefficient online inference, facing the following two problems on GPUs: (1) their high accuracy relies on the large model depth, which linearly increases the sequential computation on GPUs; (2) stochastic and dynamic online workloads cause extra costs from batching and paddings. Therefore, we present \sys for the real-world setting of GPU inference on online workloads. At its core, \sys adopts stacking distillation and boosting ensemble, distilling the original deep model into a group of shallow but virtually stacked student models running in parallel. This enables \sys to achieve a lower model depth (e.g., two layers) than the others and the lowest inference latency while maintaining accuracy. In addition, adaptive student pruning realizes dynamic student numbers according to changing online workloads. Especially for occasional workload bursts, it can temporarily decrease the student number with minimal accuracy loss to improve system throughput. We conduct comprehensive experiments to verify the effectiveness, whose results show that \sys outperforms the baselines by $4.1\times\sim 1.6\times$ in latency while maintaining accuracy and achieves up to $22.27\times$ higher throughput for workload bursts.

==> sections/artifact_description.tex <==
\section{Artifact Identification}

In this work, we present Academus to exploit student parallelism for efficient online inference of Bert-like models.
To achieve low latency and high throughput, we make the following three contributions:
\begin{enumerate}
    \item We propose student parallelism, 
	which distills the original sequential large model into a parallel group of small models 
	with the much lower model depth while preserving accuracy.
    And our artifact have implemented the training method to generate such parallel and flat student models.
	\item During the online inference, our artifact realizes special system designs for student parallelism to reduce the data parallelism
	so that waiting and irregularity can be minimized to achieve low latency and high throughput.
	\item Our artifact also realizes the adaptively dropping last-trained student models for better throughput with minimal accuracy loss
     if there is a burst in dynamical workloads.
\end{enumerate}

Generally, our artifact has two different phases for conducting experiments, including offline training and online inference.
\begin{itemize}
    \item Offline training: it trains the parallel group of students in two stages. The first stage is sequential student training. 
    It sequentially trains the group of students by boosting ensemble and virtual stacking
    to gradually mimic the original teacher to extract similar semantic representations.
    The second stage is adaptive student pruning. 
    For each training data batch, it tries to drop different numbers of last-added students to train the final classifier to realize the adaptive student pruning.
    If necessary, our artifact can distribute student models over GPUs for larger memory and higher speed. 
    \item  Online inference: we implement it in the master-worker architecture,
    employing message queues to dispatch samples and collect the results. 
    The master process is responsible for logical controlling, including resource management, the length-aware buffer, and task dispatching. 
    And workers host all concurrent student groups consisting of parallel students across different GPUs.
    We employ the Multi-Process Service (MPS) to run multiple students of different groups on the same GPUs concurrently.
    Once a user stochastically submits an inference request, the master preprocesses, buffers, and then dispatches the related samples to workers hosting the student groups for the inference. 
    During the inference, the master keeps tracking the workload intensity and occupancy of workers to adjust the student number accordingly.
\end{itemize}

With our artifact, we can reproduce various experiment results of the proposed Academus. 
Our code also contains motivation experiments to measure how different factors like model depth influence latency and throughput.
And offline training code generates the parallel group of flat student models, which can verify whether it maintains the accuracy of the teacher model.
The online inference code can reproduce the system performance results, including latency and throughput.
By removing some components and tuning parameters, it can further conduct ablation experiments.

\section{Reproducibility of Experiments}

\section{Workflow}
Overall, our experiments have three parts, including motivation experiments, offline training experiments, and online inference experiments.
We can start with the motivation experiments, which is independent of our proposed Academus to stand alone.
And Academus itself has two different phases, namely offline training and online inference.
The offline training should go first to generate the parallel group of student models for the coming online inference based on student parallelism.

\subsection{Motivation Experiments}
The motivation experiments measure the influences of different factors, including model depth, batch size, sequence length, and model number.
To prepare the experiments, we should prepare the GLUE dataset as the benchmark and pre-trained BERT models. 
And we also need to start the NVIDIA MPS as the environment preparation for the execution of multiple models.
Then we fine-tune the BERT models (including the base and the variants of different layers) on the downs-streaming tasks for coming inference.
Finally, we can run related scripts to measure how the change of different factors can affect the efficiency of model inference.

\subsection{Offline Training}
The offline training experiment generates the parallel group of flat student models equivalent to the original teacher model.
To prepare the experiments, we should prepare the GLUE dataset, the original teacher models, and the pre-trained mini BERT-like models.
Additionally, we should follow previous works to conduct data augmentation on the training data for better distillation.
For each task, we should first execute the code of sequential student training to generate the parallel group of student models'
to extract similar semantic representations with the teacher.
Then, we can execute the code of adaptive student pruning to train the final classifier with different numbers of students.

\subsection{Online Inference}
Based on student parallelism, online inference can achieve low latency and high throughput to process the stochastic online workload. 
To prepare the experiments, we should prepare the GLUE dataset and the workload trace.
And we also need to start the NVIDIA MPS as the environment preparation for multiple concurrent students on the same GPU.
After the preparation, we can start our proposed service in the master-worker architecture for online inference.

\section{Estimated Execution Time}
\subsection{Motivation Experiments}
After the proper preparation, the execution time of motivation experiments should be about one hour. 
The fine-tuning of BERT on the specific dataset should not take a long time since the size of training datasets is relatively small.
And the execution of measurement scripts for different factors should be quick.
\subsection{Offline Training}
Similar to previous works about knowledge distillation, our offline training experiments can last quite a time according to the size of the data set.
For some small datasets like MRPC, it can generate all the student models for some hours.
But it can take a long time, like one or two days, for large datasets like QQP.
And the offline training time does not affect the efficiency of the online system.
\subsection{Online Inference}
The time of online inference experiments is determined by the duration of the online workload trace. 
We can use a short duration, like one hour, to conduct this online inference experiment.
Alternatively, we can also scale the long duration into the short one.


\section{Expected Results}
\subsection{Motivation Experiments}
For each factor, our measurement scripts can measure the latency and throughput for different settings in the range.
Therefore, the script for measuring one factor can print out how the latency and throughput change with different factor values.
The execution of all measurement scripts can output the raw data to draw all four sub-figures in Figure 2 to motivate our work.
\subsection{Offline Training}
For different tasks and teacher models, we can evaluate whether the accuracy of the parallel group of flat student models can be comparable to the original teacher model.
Therefore, we can fill Table 2 in our paper by considering all tasks in GLUE and all three kinds of teacher models.
By considering different parameters (e.g., model depth and student number) and removing different training strategies (e.g., virtual stacking and pruning), 
we can conduct deep-diving experiments on the accuracy in Section 7.3.
\subsection{Online Inference}
For online inference, we can evaluate the latency and throughput of our proposed Academus.
Therefore, we can generate the related average and tail latency in Figure 7 as well as the min and max throughput results in Figure 8 in our paper.
By considering the changes of variables (e.g., model depth and student number) and adding extra inference components for data parallelism (e.g., waiting and paddings), 
we can make the deep-diving experiments about the latency and throughput in Section 7.3.

==> sections/cover_letter.tex <==
\section*{Cover Letter}

\noindent Dear KDD 25 chairs and reviewers:

It is our pleasure to have the opportunity to resubmit our revised paper "Exploiting Student Parallelism for Efficient GPU Inference of BERT-like Models in Online Services" to the Feb cycle of KDD 2025. 
We thank all the reviewers for their valuable time and constructive suggestions in the last cycle.
According to their comments, we have made several concrete revisions as follows:

\begin{itemize}
    \item \textit{Clarification on Novelty and Scope Issues.} We have revised our title, abstract, and introduction to clarify our novelty and contributions. We have more explicitly claimed that we considered a practical setting of GPU inference on stochastic workloads. Although system works have exploited parallel computing capability and handled dynamic online workloads, model design or compression works have overlooked these facts for a long time.
    As far as we know, we are \textit{the first to consider it from the view of model compression}, finding new opportunities for improvement.
    We advocate that research works on model efficiency should \textbf{make more practical assumptions to make concrete progress}. For more practical settings, we propose new \textbf{stacking distillation} to help reduce the model depth and \textbf{adaptive student pruning} for better generalization and dynamic student numbers.  
    To verify the effectiveness, we use the real-world workload trace to measure the GPU inference efficiency.
    \item \textit{Comparison with New Related Work.} Since some individual reviewers bring up some references to CNN distillation, we add them as new related work and point out the distinguished differences, such as ensemble teachers instead of students for better guidance, different branches sharing the same bottom layers, or heterogenous students suffering from serious straggler and overfitting problems. In contrast, our work generates 
    an equivalent group of homogenous, shallow, and parallel students. Virtual stacking of all students reduces the model depth to be friendly to GPU, and adaptive student pruning not only gets better generalization with fewer students but also realizes dropping students with minimal accuracy loss for workload burst.
    \item \textit{Reorganizing Methodology Section.} We have reorganized our Methodology structure to better show our novelty and technique contributions. We have added \textbf{new quantitive analysis} both on convergence and inference efficiency in this section. We also move back the length-aware buffer description from the Appendix section. We have further polished the formatting and caption of Figure 3-5 for better illustration.
    \item \textit{New Discussion Section.} We add a new section to discuss two common issues:(1) how to extend our work to generative models like GPT and the reason why we leave it as the future work; (2) the detailed training cost of our work, which is comparable to other model compression methods. 
    \item \textit{Implementation Details in Appendix.} We have added more details about the key configurations and hyper-parameters of the training procedure. Moreover, we added the detailed setting of our motivation experiments in Figure 1 in the Appendix. 
    We also moved the overall procedure of our online inference from the Methodology to the Appendix, due to the limited space.
    \item \textit{Fixed Typos and Miscellaneous.} We have fixed all the typos and grammar problems as pointed out by reviewers. Additionally, we solved some miscellaneous issues like formatting.
\end{itemize}

Please kindly refer to the following parts for our revised paper. And we are looking forward to your feedback.
We would like to thank all chairs and reviewers for your time and efforts in reviewing and organizing KDD 2025 again! 
~\\
\noindent Best Regards

\noindent All the Authors of Submission \#2326  

==> sections/design_backup.tex <==


\section{Model Decomposition and Parallelization}

\subsection{Architecture Overview}
\begin{figure*}[ht]
	\centering
	\includegraphics[width=\textwidth]{figures/overview.pdf}
	\caption{Overview of \sys in the two phases: (1) training phase: design new model distillation algorithm converting the teacher model into a group of student models; (2) inference phase: employ multi-queue to dispatch small data batches in similar sequence lengths and manage the resource allocation by adjusting the number of student models}
	\label{fig:overview}
\end{figure*}
\sys actively generates the group of flat models explicitly working together,
rather than passively selecting on-the-shelf models for bagging ensemble. 
\begin{comment}
 In the style of boosting ensembles, 
 \sys proposes a novel knowledge distillation algorithm to transfer the knowledge of the deep teacher into a group of student models, which imitate different layers of the original teacher. 
During the inference, all student models run in parallel to fully utilize parallel computation resources. 
\end{comment}
As the architecture overview shown in Figure~\ref{fig:overview},  \sys consists of two different phases:
\begin{itemize}
	\item  \textbf{Training phase}: \sys applies the idea of boosting ensemble to distill the deep teacher model into multiple student models equivalent to the original model.
	It sequentially trains student models to gradually reduce the error between the teacher and all students. 
	More importantly, \sys makes different students to imitate different layers of the teacher in their intermediate layers for better diversity and generalization of the ensemble.
	
	\item \textbf{Inference phase}: To serve the group of student models for stochastic workloads,
 \sys employs the specialized mechanisms of resource management and task dispatching during inference. 
 It distributes different students over different GPUs and duplicates each student multiple times on the same GPU. 
 \sys also uses the "merging queue" to merge the samples of the same length into small batches 
 and then dispatch the individual samples or small batches to run concurrently instead of large and regular batches. And it can adjust the student number according to the variance of stochastic workloads.


\end{itemize}

\subsection{Training Phase}

\begin{comment}
Although attention-based models rely on the deep architecture for hierarchical representation learning like any deep models, the inference latency linearly increases with the model depth, which is critical for time-sensitive applicatins. 
Since all student models can be computed in parallel on massive GPUs, multiple flat students essentially trade more parallel operators for fewer serial operators. 
To reduce the latency, every student model shares the same model architecture that has much fewer attention blocks than the teacher. 
All flat student models work together in the way of boosting ensemble to better imitate the teacher's output and maintain the accuracy.
	


\begin{figure}[t]
	\includegraphics[width=0.5\textwidth]{figures/MD_flow.pdf}
	\caption{The flow of model decompostion}
	\label{fig:model_decomposition}
\end{figure}
\end{comment}

\begin{algorithm}[ht]
\caption{Model decomposition pseudo code}
\label{algo:boosting}
	\begin{algorithmic}
		\REQUIRE TeacherModel, PreMiniModel, threshold
		\STATE \textbf{\#Students Generation:}
		\STATE	studentList = [PreMiniModel]
		\REPEAT
			\STATE	\#Initialize current student
			\STATE  student= studentList[-1].copy()
			\STATE	\# Sample the data of the largest differences in the final representation of the teacher
			\STATE 	dataloader = residualSample()
			\STATE  \# train the new student on sampled data to virtually stack on previous students and gradually correct the errors
			\STATE  student = train(student, dataloader)
		\STATE  studentList.append(student)   
		\UNTIL 	len(studentList) > threshold
		\STATE 	studentList = studentList[1:]
		\STATE
		\STATE \textbf{\#Adaptive pruning and combination of students}
			\STATE \# Generate soft label from the teacher
			\STATE softLabel=TeacherModel(x)
			\STATE \# Adaptively sum up previous $k$ students to train the student classifier on the soft label.
			\STATE adaptiveTrain(studentList, classifier, softLabel)
			\STATE \# prune the student number to get the best accuracy
			\STATE pruneEnsemble(studentList, classifier)
	\end{algorithmic}
\end{algorithm}

Following the rationale mentioned above, \sys gradually decompose the large PLMs into an equivalent group of flat student models through knowledge distillation. 
As illustrated in Algorithm~\ref{algo:boosting}, there are two stages to realize the model decomposition:
\begin{enumerate}
 \item \textbf{Student models generation}: \sys sequentially trains multiple student models in the style of boosting ensemble to extract the final representation similar to the original teacher model. 
Each student learns to distill different layers of the teacher into its intermediate layers to realize model decomposition and improve accuracy.
\item \textbf{Adaptive student model combination and pruning}: it dynamically sums up different numbers of students as the final representation to train the classifier under the guidance from the teacher. Finally, the student number is pruned for the best accuracy in case of overfitting, and it can be further reduced with minimal accuracy loss.
\end{enumerate}

 


\subsubsection{Student Models Generation}

Now we introduce how \sys trains the multiple flat student models explicitly working together to extract similar  representations to the teacher model.
According to the theory of ensemble learning, different weak models need significant diversities to improve accuracy.
Since all student models share the same network architecture, we design the novel training algorithm to improve diversities from other aspects, including training objects, parameter initializations, and data sampling.

To achieve diversity, \sys applies different training loss functions to different student models. 
All students are sequentially trained in the style of boosting ensemble to correct the residual error on the final representation gradually. 
Except that the first student directly imitates the teacher, other students learn to correct the error of previous students. Formally, the training loss of the i-th student $L_1^{(i)}$  is shown in the following equation:
	\begin{equation}
		L_1^{(i)}(x)= 
	\begin{dcases}
		\left\| T(x)-S^{(i)}(x)) \right\|^2, & i=0 \\
		\left\| T(x)-\sum_{j=0}^{i-1}\alpha_j S^{(j)}(x)-S^{(i)}(x) \right\|^2 , & i>0 .
	\end{dcases}
	\end{equation}
	In the equation, the $T(x)$ stands for the final representation output of the teacher model. $S^{(i)}(x)$ denotes the final representation of the i-th student model. $\alpha_j $ is the shrinkage rate for the j-th student in the boosting ensemble, in which we have $\alpha_0 = 0$ and any other $\alpha_j \in (0,1) $. In this loss, only $S^{(i)}$ is trainable, while the other models like $T$ and $S^{(j)}$ are fixed.

Despite that all students run in parallel, \sys proposes the stacking distillation to make every student virtually stacked on the previous students. Any student learns to distillate the ensemble of all previous students into the representation of its $N/2$-th layer. Since stacking distillation makes the intermediate representation imitates all the previous students, the following layers can better correct the error by refining the intermediate representation. The loss $L_2^{(i)}$ of stacking distillation for the i-th student is defined as follows:
	\begin{equation}
		L_2^{(i)}(x) = \left\| \sum_{j=0}^{i-1}\alpha_j S^{(j)}(x)-M^{(i)}(x) \right\|^2
	\end{equation}
	where $M^{(i)}(x)$ denotes the intermediate representation of the $N/2$-th layer in the i-th student model. In this loss, only $M^{(i)}$ is trainable while the other models are fixed.
	
	Therefor, the overall training loss $L$ for the whole representation imitation can be written as follows:
	\begin{equation}
		L=L_1+\lambda L_2
	\end{equation}
	where $\lambda$ is the hyper-parameter to balance the final representation distillation and stacking distillation.


Besides the different training loss, \sys also brings in diversities by initializing the parameters of student models in different ways.
The first student is initialized with a pre-trained language model to improve the generalization, 
while any other student copies the parameters from the last trained student for the initialization. 

Additionally, every student model is trained on different sampled subsets of training data, except only the first student is trained on the whole training data. For any student, we pick up the top $a\%$ samples with the largest residual errors between the teacher and the existing students. And we randomly sample another $b\%$ of all the training data in the rest part. And the subset of training data is augmented in the way suggested by previous works~\cite{jiao2019tinybert,hou2020dynabert}.
%one by one to gradually reduce the final representation differences between the teacher and the all students. 
\begin{comment}
Before training the student model, we use pre-trained compact model to initialize the student to improve the generalization. 
And we prepare a subset of the training data that has large residual errors. 
The final representation layer of every student is trained to correct the error of all previous students, while the intermediate layer learns to intimate the final outputs of all previous students.
Specifically, we present the details of student training as follows:
\end{comment}

\subsubsection{Adaptive Pruning and Combination of Students} 
\begin{algorithm}[t]
\caption{Pseudo code for adaptive training and pruning of students}
\label{algo:classifier}
	\begin{algorithmic}
		\REQUIRE TeacherModel, studentList, Classifier, Dataset
		\FOR{batch in Dataset}
			\STATE softLabel = TeacherModel(batch)
			\FOR{k in range(len(studentList))}
				\STATE rep=$\sum_j^{k}\alpha_j studentList[j](batch)$
				\STATE output = Classifer(rep)
				\STATE loss = softCrossEntropy(output,softLabel)
				\STATE Accumulate the gradients of current k students
			\ENDFOR
			\STATE Update the classifier and all students according to the accumulated gradients
		\ENDFOR
		\STATE Prune the number of student models in the ensemble according to the test performance for better generalization
	\end{algorithmic}
\end{algorithm}
After training the group of student models to output final representations similar to the teacher's, \sys further learn to imitate the final output of the teacher. 
We put a new classifier layer on the sum of the students' outputs, which brings in quite limited communication costs thanks to the small size of student outputs. 
And we take the soft labels outputted from the teacher model as the target in the soft cross-entropy loss instead of hard labels of the ground truth. 

During the training,  we sample different student numbers $k$ to generate the final classifier layer's final representation in one training data batch. 
There are two reasons for it: one is to prune the students of the ensemble to improve generalization in case of overfitting~\cite{margineantu1997pruning,wu2021boosting}; the other is to realize the adaptive number of students in the inference.
Since the tail students try to correct the error of the previous ones, we always pick up the previous $k$ students to generate the final representation.
We conduct the forward and backpropagation on different numbers of students and accumulate the gradients of different student numbers to update the parameters of the classifier and students. 
We present the detailed algorithm for the classifier distillation in Algorithm~\ref{algo:classifier}.


\begin{comment}
\subsubsection{Diversity Analysis}
According to the theory of ensemble learning, the diversity of different models determines the generalization performance of the ensemble. If different models are more irrelevant with each other, then the failure probabilities of different models are more discorrelated and even independent. Therefore, if we give the same input to multiply models of high diversity, the overall failure probability of the ensemble can decrease exponentially with the model number. 

In this work, we leverage the boosting ensemble to train multiple distillated students. Although all student models share the same network architecture, we bring in the diversity to improve generalization in the following aspects:
\begin{itemize}
	\item \textbf{Model Initialization:} We initialize different student models in different ways. The parameters of the first student model is initialized with the pre-trained compact models. And any other student model copy the trained parameters of the previous student as its initial parameters. Therefore, all student models have different initial parameters, despite of the same network architecture.
	\item \textbf{Data Subsampling:} We subsample different subsets of training data for different students. The first student is trained on the whole training data set. However, the rest students pick a part of data samples according to the residual errors of its previous students.
	\item \textbf{Training Loss:} We train the student models on the different losses. In the final layer, every student learns to correct the error of its previous students. And in the intermediate layer, every student distillates the ensembled final representation of previous students into its intermediate representation. 
\end{itemize}
\end{comment}

\subsection{Inference Phase}
In the inference phase, we make a specialized system design to make \sys directly process the stochastic arrived samples instead of accumulated data batches. As shown in the right part of Figure~\ref{fig:overview}, the inference process has the following steps: 
(0) In the initialization, resource management distributes all student models over different GPUs, and every student is replicated on the same GPU to process different samples concurrently; 
(1) users submit inference requests; 
(2) the inference request is buffered in the merge queue according to different sequence lengths; 
(3) If a set of student models is available, the dispatcher assigns the data sample or a small batch of the same length to them for inference; 
(4) Resource management adjusts the number and allocation of student models according to the workload changes. 

\subsubsection{Resource Management}
In the initialization of the inference service, the resource management distributes the whole set of model batches across different GPUs to make better use of massive GPUs in the cluster. 
The models distributed across different GPUs can have not only more parallel computation power but also higher GPU memory bandwidth to access the intermediate results and model parameters.
If we allocate the whole model batch in the same GPU, the models running in parallel on the same GPU can have more GPU memory access conflicts than the distributed allocation, despite the abundant computation resources for small data batches.

We also host different model batches on the same set of GPUs for better utilization. 
Because a single or a small batch of inference samples cannot fully utilize the high parallel computation of the GPU, we can start multiple model inference processes to wait for any newly arrived inference requests. 
Different inference samples do not arrive at the same time. The same set of GPUs can process them in the form of a pipeline to avoid memory conflicts between different samples. 
Therefore, \sys can concurrently process different data batches to better utilize parallel computation capability but less memory access conflicts.

During the inference service, resource management can adjust the number of student models according to the intensity of the real workload. 
Resource management can reduce the student number by dropping the student models in the tail if the workload is too heavy. According to the boosting ensemble, it can trade minimum accuracy for larger system throughput. And if the workload tends to be light, it can increase the student number for better prediction quality.
We estimate the inference sample number of \sys to process concurrently in different settings of student numbers by profiling.

\subsubsection{Merging Queue}
\begin{figure}[t]
\centering
	\includegraphics[width = \linewidth]{figures/merge_queue.pdf}
	\caption{Merge Queue: Newly arrived sequence sample (e.g., the red one whose length is 64) can be merged with the previous element if their lengths are the same. Otherwise, the new sequence sample (e.g., the blue one whose length is 30) is added to the queue's tail. }
	\label{fig:multi_queue}
\end{figure}
After the inference request arrives, \sys buffer it in the merging queue according to its sequence length in the scenario of interactive inference.
In the data preprocessing, we parse the character string into a token sequence and convert all tokens into token IDs. 
After counting the sequence length, we only clip the sequence if it is over the maximum length, but we do not pad any short sequence as in the previous works. Then we enqueue the preprocessed data sample into the merging queue, which buffers the sequences according to not only the order but also the length. 

As shown in Figure~\ref{fig:multi_queue}, the element of the merging queue can either be a single sample or a small data batch of the same length. We set the length and queue position as the key-value pair in the dictionary to record the queue position of different sequence lengths. When a new data sample arrives, we check the dictionary to see if there is any sequence of the same length in the queue. If so, we can get the position from the dictionary and merges the new sample with the existing ones into a small data batch. Otherwise, we just put the new sample in the tail of the queue and add its length and position in the dictionary. When a sample or small data batch comes out of the queue, we also delete its key-value pair in the dictionary and deduct the position values of other keys by one.



\subsubsection{Dispatcher} 
If the merging queue is not empty, the task dispatcher schedules the inference samples to execute on the proper set of student models immediately. In general, the dispatcher assigns the different dequeued data samples or batches to different sets of student models to run concurrently other than the data parallelism of the data batch. To balance the workloads, we arrange the inference samples to run on different student sets in the round-robin way. Therefore, a set of GPUs hosting multiple sets of students can concurrently process multiple inference samples arrived at different times. As a result, the concurrent inference samples can share the memory access bandwidth in different time slices and fully utilize all the computation resources of the GPU. Once the inference on the data sample or batch is finished, the results are returned to the dispatcher and then returned to users.

During the inference service, the dispatcher keeps tracking the intensity change of the workload and the status of resource usage to notify resource management about the adjustment. To estimate the intensity of workload, it counts the elements waiting in the merging queue for the inference. And it also records the amount of incompleted inference samplers running on all GPUs. If the number of waiting samplers has been larger than the capability of the current setting of \sys, the dispatcher notifies the resource management to decrease the student number to be small enough to concurrently process all samples in the queue. And if the merging queue is empty and the number of samplers running on GPUs is always smaller than the threshold for a certain time, the dispatcher asks the resource management to increase the student number for better accuracy and higher utilization.


\begin{comment}
To fully utilize the GPU cluster to process the practical workloads, we make specialized system design in resource management and task dispatcher for the model batch inference.  
\name explicitly takes the practical workloads, namely stochastically arrived requests of different sequence lengths, into the consideration of system design. 
It aims to conduct inference on continuous small batches or even single requests with low latency and high utilization of the GPU cluster, instead of accumulated large data batches.
In general, \name conduct the model batch inference of single or a small batch of requests on a set of GPUs to improve parallelism and reduce the memory conflictions. And different small batches can conduct con-current inference on the same set of GPUs to further improve device utilization with the pipeline.
Specifically, the model inference system consists of three key components including resource management, merging queue, and dispatcher, which are discussed in details later.
\end{comment}




%it aims to schedule inference requests to execute on GPUs as soon as possible. It usually dispatch the small data batch or even single sample if resources are available. To overlap the transfer time and improve device utilization, it can schedule different small data batches to con-currently run on the same GPUs. 
%\subsubsection{Analysis}
%aa

==> sections/design_v2.tex <==
\begin{figure*}[ht]
	\centering
	\includegraphics[width=\textwidth]{figures/overview.pdf}
	\caption{Overview of \sys in the two phases: (a) training phase: design new knowledge distillation converting the teacher model into a group of student models for student parallelism; 
	(b) inference phase: specialized system design for student parallelism, including model allocation for workers, length-aware buffer, and student number adaptation.}
	\label{fig:overview}
\end{figure*}

\section{Design V2}

\subsection{Architecture Overview}
To achieve low latency and high throughput, \sys adopts the student parallelism with the group of parallel student models. 
It trades more parallel operators in multiple students for less serial operators among layers while maintaining accuracy. 
%It proactively trains the group of student models for explicit boosting ensemble, so that all student models have the flat, decoupled, and homogenous architecture friendly to GPU parallel computing.
As the overview in Figure~\ref{fig:overview},  \sys consists of two parts: the online part and offline part. 
In the offline part, it proactively generates a group of parallel students equivalent to the teacher for high accuracy, 
while having flat, decoupled and homogenous architectures friendly to GPU acceleration.
And in online inference, \sys has specialized system mechanisms for student parallelism to replace data parallelism for stochastic workloads and irregular lengths,
like distributed model allocation and length-aware queue. 
Moreover, it further conducts adaptive pruning to drop some students with minimal accuracy loss to handle workload burst.

\subsection{Offline Generation of Parallel Students}

\begin{comment}
	
\begin{figure}[t]
	\includegraphics[width=0.5\textwidth]{figures/MD_flow.pdf}
	\caption{The flow of model decompostion}
	\label{fig:model_decomposition}
\end{figure}
\end{comment}

\begin{algorithm}[t]
\caption{Training students for student parallelism}
\begin{algorithmic}
\Require TeacherModel, PreMiniModel, StudentNum
\State \textbf{\#Sequential training of student models}
\State studentList = []
\For {$i \gets 1$ to StudentNum}
	\State newStudent = PreMiniModel()
	\While {training}
		\State outputs\_t = TeacherModel(x)
		\State outputs\_s = newStudent(x)
		\State Compute the losses as Equation~\ref{equ:boost} and Equation~\ref{equ:layer}
		\State Update the newStudent
	\EndWhile
	\State studentList.append(newStudent)
\EndFor
\State \textbf{\#Combination of stuent models}
\While{training}
	\State softLabel = TeacherModel(batch)		
	\State rep=$\sum_{j=0}^{\text{StudentNum}}\alpha_j studentList[j](batch)$
	\State output = Classifer(rep)
	\State loss = softCrossEntropy(output,softLabel)
	\State Update the classifier and all students
\EndWhile
\end{algorithmic}
\label{algo:boosting}
\end{algorithm}
 

In general,
\sys distills the LLM into an equivalent group of parallel student models working in explicit boosting ensemble, 
inspired by the residual connections in LLM (implicit boosting ensemble). 
Since all student models have the same flat architectures, it is challenging to maintain the accuracy for those weak and homogenous students.  
As described in Algorithm~\ref{algo:boosting}, \sys has two stages to train the group of parallel students to solve the problem:
\begin{enumerate}
	\item \textbf{Sequential student training}: Inspired by boosting ensemble, \sys sequentially trains all students to generate the final representation together. 
	For high accuracy, different flat students are trained on different losses to improve the ensemble diversity. 
	%Different students distill different layers of the teacher into its intermediate layer.
	%And every student learns to reduce the residual error on final representation between the teacher and its previous students. 
	
   \item \textbf{ Combination of students}: It further trains the final classifier layer on top of the ensemble of all students. 
   And the teacher generates soft label to guide the simultaneous training of the final classifier and all students.
   \end{enumerate}

\subsubsection{Sequential Training of Student Models}
According to ensemble learning theory, different weak models need significant diversities to improve generalization and accuracy~\cite{zhou2021ensemble}.
Since all student models share the same flat and pre-trained network (e.g. 2 layers) for student parallelism, 
we design novel training losses that are different for all student models instead of the different network architectures.
It makes different students learn different levels of knowledge from the teacher in layer distillation. 
And it sequentially trains student models to gradually reduce the residual error on final representation between the teacher and its previous students.
%In this subsection, we introduce how \sys trains the multiple flat student models in parallel, 
%which explicitly work together to extract similar representations to the teacher model.

Specifically, we propose layer distillation to distill different layers of the teacher into different student models as their regularization on intermediate layers. 
Therefore, different student models can reserve different levels of hierarchical semantic representations from the implicitly ensembled teacher.  
For example, the $i$-th student distills the $(N/2+i)$-th layer of the teacher into its intermediate layer. 
The objective function $L_2^{(i)}$ of layer distillation for the i-th student is defined as:
	\begin{equation}
		L_1^{(i)}(x) = \left\| T_{(\lfloor N/2 \rfloor+i)}(x)-M^{(i)}(x) \right\|^2
	\label{equ:layer}
	\end{equation}
	where $M^{(i)}(x)$ denotes the intermediate representation of the middle layer in the i-th student model. $T_{(\lfloor N/2 \rfloor+i)}(x)$ is the output of $N$-th layer from the teacher. In $L_2^{(i)}$, only $M^{(i)}$ is trainable while the $T_{(\lfloor N/2 \rfloor+i)}(x)$ are fixed.
	
Furthermore, different student models have different residual errors to correct on their final layer to gradually improve accuracy.
Although all students are in parallel for the inference, every student is sequentially trained in the style of boosting ensemble.
Namely, every newly added student is trained to further reduce the residual error between the teacher and its previous students. 
Except that the first student directly imitates the teacher, other students learn to correct the error of previous students. Formally, the training loss of the i-th student $L_1^{(i)}$  is shown in the following equation:
	\begin{equation}
		L_2^{(i)}(x)= 
	\begin{dcases}
		\left\| T_{(N)}(x)-S^{(i)}(x)) \right\|^2, & i=0 \\
		\left\| T_{(N)}(x)-\sum_{j=0}^{i-1}\alpha_j S^{(j)}(x)-S^{(i)}(x) \right\|^2 , & i>0 .
	\end{dcases}
	\label{equ:boost}
	\end{equation}
	In the equation, the $T_{(N)}(x)$ stands for the output of $N$-th teacher layer, i.e., the final representation output of the teacher model. $S^{(i)}(x)$ denotes the final representation (e.g., the second layer) of the i-th student model. $\alpha_j $ is the shrinkage rate for the j-th student in the boosting ensemble, in which we have $\alpha_0 = 0$ and any other $\alpha_j \in (0,1) $. Only $S^{(i)}$ is trainable, while the other models like $T$ and $S^{(j)}$ are fixed.


	Therefor, the overall training loss $L$ for the i-th student can be written as follows:
	\begin{equation}
		L=\lambda L_1+ L_2
	\end{equation}
	where $\lambda$ is the hyper-parameter to balance layer distillation and final residual error correction.
	And the total student number is determined by the model depth of the teacher because of different layer distillation.

\subsubsection{Combination of students}
After all students are trained to generate final representation together to be similar with the teacher's, 
\sys further learns to imitate the final output of the teacher.
We sum up the final representation of all students as the combination to feed the final classifier layer, 
which has quite limited communication costs thanks to the small size of the pooled final representation. 
To better guide the training, we take the soft labels generated by the teacher model as the target in the soft cross-entropy loss rather than the hard labels of the ground truth. 
And we go through the whole dataset of the downstreaming task to train or finetune the final classier layer and all students together.


\subsection{Online Inference in Student Parallelism}
During the online inference, \sys makes specialized system designs for student parallelism to avoid data parallelism for the practical online workloads.
 As shown in Figure~\ref{fig:overview} (\emph{right}), the inference in student parallelism has the following procedures: 
 (i) In the initialization, the resource manager distributes and replicates student models to start concurrent workers;
 (ii) A new inference sample is submitted; 
 (iii) The new sample is preprocessed and stored in the length-aware buffer; 
 (iv) If any worker is idle, it dispatches the first buffered sample or a small batch of the same length for the inference; 
 (v) If the buffer is full or enough workers are idle, resource management decreases the student number for larger throughput or increases it for better accuracy (details in \S~\ref{sec:adaptiv_pruning}); 
 (vi) It returns results back to users. 
 
\subsubsection{ Inference on Concurrent Samples}
To get rid of the waiting queue and paddings, \sys employs student parallelism to replace data parallelism.
Therefore, it exploits the parallel structures of student models to directly dispatch individual samples instead of data batches for the inference.
% \sys free of computation dependency for better parallelization. 
It starts multiple concurrent workers to handle different samples respectively,
because each worker runs on its own group of student instances.

In the initialization, the resource management distributes all student models of one worker across different GPUs to make fully use of massive GPUs in the cluster. 
The models distributed over different GPUs can have not only more parallel computation power but also higher GPU memory bandwidth to access the intermediate results and model parameters.
If we allocate student instances of one worker on the same GPU, they can access the memory simultaneously to cause more memory conflicts despite the abundant computation resources.

Additionally, \sys replicates every student model for multiple instances on its GPU for different workers to better utilize the single GPU.
Because a single or a small batch of inference samples cannot feed up the GPU's high parallel computation capability, 
we can host multiple model instances of different workers to concurrently process inference requests arriving stochastically. 
Since different inference samples do not arrive at the same time, 
the same set of GPUs can process them in the pipeline to overlap PCI-E transferring and memory accessing. 
Therefore, \sys can concurrently process different samples to better utilize parallel computation capability but less memory access conflicts.

\subsubsection{Length-aware Buffer}
\begin{figure}[t]
\centering
	\includegraphics[width = 0.9\linewidth]{figures/length_aware_buffer.pdf}
	\caption{Length-aware Buffer: Newly arrived sequence sample (e.g., the red one whose length is 64) can be merged with the previous element into a small batch, if their lengths are the same. 
	Otherwise, the new sequence sample (e.g., the blue one whose length is 30) is added to the buffer's tail. }
	\label{fig:multi_queue}
\end{figure}

\sys employs the length-aware buffer to merge the samples of the same length for better throughput.
Once the inference sample arrives, we preprocess it to clip the long sequence into the maximum length.
If the length-aware buffer is not empty, it tries to merge the samples of the same length into a small data batch as one buffered element on the fly.
Whenever any worker is idle, the dispatcher immediately sends out the first element in the buffer for the inference.
And we set the maximum buffer size as the total number of current workers, 
so the range of buffer time is from zero to the inference latency.

Figure~\ref{fig:multi_queue} shows the details about how a length-aware buffer generates small batches of the same length.
We set the sample length and pointer as the key-value pair in the dictionary to quickly index samples of different sequence lengths. 
When a new sample arrives, we check the dictionary to see if any sample has the same length in the buffer. 
If so, we can get the pointer from the dictionary and merge them into a small data batch as one element in the buffer. 
Otherwise, we append the new sample as the tail element in the buffer and add its length and pointer in the dictionary. 
When a sample or small data batch is dispatched, we delete its key-value pair in the dictionary.


\subsection{Adaptive Pruning for Student Parallelism}
\label{sec:adaptiv_pruning}
\begin{algorithm}[t]
	\caption{Adaptive pruning for student parallelism}
	\begin{algorithmic}
	\Require TeacherModel, StudentList, StudentNum
	\While{training}
		\State softLabel = TeacherModel(batch)		
		\For {$k \gets 1$ to StudentNum}
			\State rep=$\sum_{j=0}^{k}\alpha_j studentList[j](batch)$
			\State output = Classifer(rep)
			\State loss = softCrossEntropy(output,softLabel)
			\State Accumulate the gradients of current k students 
		\EndFor
		\State Update all parts based on the accumulated gradients
	\EndWhile
	\For {$k \gets 1$ to StudentNum}
			\State evaluate the previous $k$ students on validation set
	\EndFor
	\State Choose the best previous $n$ students
	\end{algorithmic}
	\label{alg:adaptive_pruning}
\end{algorithm} 
According to Occam's Razor, pruning can remove the redundant parts of trained model and improve accuracy of remained parts (better than directly training the small remained parts). 
Since the newly added students of boosting ensemble marginally improve accuracy by reducing the residual error, 
we can drop last-trained students for pruning to realize computation reduction with minimal accuracy loss.
Moreover, pruning the students in the ensemble can also further improve generalization in case of overfitting~\cite{margineantu1997pruning,wu2021boosting} in large scale ensemble. 
Specifically, adaptive pruning of students dynamically sample different student numbers when training the final classifier. 
During the training of one data batch, 
we dynamically drop different $k$ last-trained students to generate the final representation for the classifier training as described in Algorithm~\ref{alg:adaptive_pruning},
which can replace the stage 2 in Algorithm~\ref{algo:boosting}. 
We conduct multiple forward and back propagations on different numbers of students for the same training data batch. 
And it accumulates all the gradients to update the parameters of the classifier and all students. 

During the inference, 
the resource management dynamically adjust the student number to host different numbers of workers according to the workload intensity and resource usage.
%If workload burst occurs, \sys can reduce the student number to start more workers for better throughput.
It keeps tracking the buffer size and idle worker number as the indicators of workload intensity and resource usage. 
If the buffer size reaches the threshold (e.g. 80\% of total worker number), 
\sys drops some last-trained student models to start enough workers that can handle all buffered samples. 
And if over a quarter of workers are idle and the length-aware buffer remains to be empty for a certain time window (e.g. 2 minutes), 
then it improves the student number to makes full use of computation resources to achieve better accuracy.
To avoid cold starting for the entire environment, 
the inactivated workers of different student numbers can wait in the host memory to realize hot standby.



==> sections/discussion.tex <==
\begin{comment}
\section{Related Work}
There have been various efforts to improve the inference efficiency of LLMs, 
but they all do not directly reduce the serial computation costs and cannot be flexible to handle the dynamic changes in workloads and requirements. We can classify all previous works into two categories: model optimization and system optimization.
\subsection{Model Optimization} 
All previous model optimization works cannot reduce the model depth to the two layers without significant accuracy loss. 
These model optimization usually aims to enable the deployment on edge devices with limited computation and storage capabilities instead of the powerful GPU cluster.
Therefore, they focus on reducing proxy metrics like total Flops and model size instead of directly optimizing the wall time of the inference.
They also assume that regular sample data batches are available for inference just like training and overlook the stochastics of actual workload in arriving patterns and sequence lengths. 
 Specifically, there are several algorithm approaches as follows:
 
\begin{itemize}
\item \textbf{Quantization:} These works~\cite{kim2021bert,bai2020binarybert,shen2020q} attempt to replace the expensive float parameters and calculations with cheap low-bit integral ones. Quantization makes every parameter smaller and every operator quicker, but the dependency and the number of total operators do not decrease. Although the quantized model is more friendly to weak edge devices, it cannot decrease the serial and overall computation complexity and fails to better utilize the high-end parallel computation devices in data centers. 

\item \textbf{Pruning:} According to the lottery theory~\cite{chen2020lottery}, some works~\cite{DBLP:conf/rep4nlp/GordonDA20,michel2019sixteen, hou2020dynabert} prune the redundant weights or structures like attention heads or even layers to reduce the model parameters. Although these works save some memory and total computation without hurting the accuracy, they can only reduce the model depth to a limited degree, like six layers, to maintain the accuracy, far away from the minimum number, like two layers. And most works in this line overlook the chance to improve the model width and take advantage of parallel computation capabilities. SensAI~\cite{wang2021sensai} tries to split a mutli-class model into several pruned networks responsible for predicting different classes, but it is not suitable for popular regression(e.g., ranking) and binary classification(e.g., Sentiment or similarity classification) tasks in NLP. 
%More importantly, SensAI pruned different models for different classes resulting in inference on irregular models.
  
\item \textbf{Knowledge distillation:} Some other works~\cite{sanh2019distilbert, sun2019patient, jiao2019tinybert} train a small student model from the guide of the original teacher model. The student models usually have fewer layer numbers, but they still cannot maintain accuracy with only two attention-based layers. They also assume a large data batch available for inference and leave the problem of stochastical workloads in practice unsolved. Compared with our work, all previous knowledge distillation works are limited to learning only one student model. However, our work explores more rooms to further reduce the layer number by generating a batch of flat students.

\item \textbf{Adaptive computation:} These works~\cite{DBLP:conf/acl/XinTLYL20, DBLP:conf/acl/LiuZWZDJ20,zhou2020bert }  add an output classifier for every layer to realize dynamic inference, so that some easy data samples can early exit from the bottom layers. However, other hard samples still have to go through more or even all layers, resulting in high tail latency. Worse, these works also ignore the stochastics of real workload and suffer from inefficiency in practice. 

\end{itemize}

\subsection{System Optimization}
Some existing inference systems have tried to solve the problems caused by the stochastics of real workloads in both arriving patterns and sequence lengths, but they bring in extra idle waiting time and resource wasting. Specifically, they have made some attempts to employ techniques as follows:
\begin{itemize}
\item \textbf{Waiting Queue and Sequence Padding:} System works~\cite{zhang2019mark, ali2020batch, gunasekaran2022cocktail} employ waiting-queue and sequence padding to form large and regular data batches for better throughput and device utilization. However, the patterns of request arriving change over time, and there are even some sudden changes like bursty~\cite{khaleq2018cloud}. Therefore, it is hard to always make quick and correct decisions to set the proper batch size and waiting time threshold~\cite{khaleq2018cloud, ali2020batch}. And short sequences need paddings to form the regular data batch, resulting in extra time and space costs. But our work can directly dispatch samples to run on a group of models instead of data batches.
%\item \textbf{Sequence Padding:} To run in batches on GPU, inference systems~\cite{romero2021infaas, crankshaw2017clipper, gunasekaran2022cocktail} have to pad the sentences in the natural language into sequences of the same length. However, shorter sequences have to pay the same time and space cost as the longest or maximum length in the same batch. The padding not only brings in the extra storage space but also additional computation complexities in the attention-based layers. However, \sys do not need any paddings to form regular data batches for the data parallelism.
\item \textbf{Model Selection for Bagging Ensemble}: Existing system works~\cite{crankshaw2017clipper, gunasekaran2022cocktail}  also attempts to select and ensemble some cheap models from all model candidates to reduce inference latency. However, the simply bagging ensemble of such on-the-shelf models has limited potential to decrease the latency and improve the accuracy. Worse, the selected models have different network architectures and inference time, leading to extra idle waiting. In contrast, our work generates flat and homogenous student models to explicitly work together to trade more width for less depth.
\item \textbf{Resource Scaling:} Some other inference systems~\cite{gunasekaran2022cocktail, yang2022infless} explore auto-scaling in resource management to handle the bursty workloads. However, due to the unpredictable intensity of workloads, they can have over-provision on reserved computation devices, resulting in resource wasting. And they can also wait a long time for the cold starting of new nodes or even be out of new resources if an unexpected heavy workload happens. But our \sys can decrease the student number to improve the throughput with the given resources.
\end{itemize}
\end{comment}

\section{Discussion}

\textbf{Generality.} %Although our work and experiments focus on the NLP tasks, 
%it has the potential to a general inference solution for other fields using the large attention-based models.
Besides the field of NLP, BERT-like models are more and more popular in various fields. 
For example, BERT-like models have shown strong performance on tabular data problems in data mining~\cite{gorishniy2022embeddings}. 
Vision Transformers (ViTs)~\cite{DBLP:conf/iclr/DosovitskiyB0WZ21} takes patches of one image as the tokens to feed BERT-like models, 
which have achieved the state-of-the-art accuracy for image classification and segmentation.
CLIP~\cite{DBLP:conf/cvpr/LiXWZ0Z0JC22} employs attention layers to connect text and images to realize effective multi-modality learning.
%And Graph Attention Networks~\cite{velivckovic2017graph} replace graph convolution with attention mechanism on graph data.
Because all these works share the same architecture of stacked attention layers with residual connections, 
our method can also be extended to solve different problems from these fields. 
And we leave the extension as our future work due to limited space.

\textbf{Training Cost.} Our offline training phase have similar time cost with other model training optimizations.
Although we need to train multiple students, the student is a much smaller model compared with the teacher. 
And each student is trained on the sub-sampled dataset based on the residual error in the boost ensemble learning.
We can also use distributed training on multiple GPUs to speed up.
Generally, \sys has similar level of offline training cost with previous distillation works. 
Furthermore, offline training cost does not affect the online inference at all. 
And the training cost can be amortized during the long-term deployment.

\textbf{Orthogonal Works.} 
There are some other related works orthogonal to \sys.
Quantization and mixed-precision~\cite{kim2021bert,bai2020binarybert,shen2020q} attempt to replace the expensive float parameters and operators with cheap ones,
but it does not reduce either serial computation dependency or the total operator number.
Some works~\cite{DBLP:conf/nips/ZaheerGDAAOPRWY20} focus on reducing the computational cost of the attention for the long sequence.
Tensor compilers~\cite{chen2018tvm,DBLP:conf/mlsys/FegadeCGM22} take specific models into consideration to generate optimized code on diverse DL hardware for efficient execution.
DVABatch~\cite{DBLP:conf/usenix/Cui00WLZ0G22} proposes the multi-entry multi-exit batching for better instruction scheduling on GPUs. 
DeepSpeed~\cite{DBLP:conf/sc/AminabadiRALLZRSZRH22} employs bottom optimization in operators and memory accesing.
Our work can be further combined with those works.

\begin{table}[t]
	\small
	\begin{tabular}{c|cccc}
	\hline
	Node\#(GPU\#)              & 1(4)           & 2(8)           & 3(12)          & 4(16)           \\ \hline
	%Throughput (ratio) & 15836.2 (1.00) & 31471.5 (1.99) & 46853.5 (2.96) & 62789.3 (3.96) \\ \hline
	Throughput & 15836.2 & 31471.5  & 46853.5  & 62789.3  \\ 
	ratio 	   & 1.00    & 1.99     & 2.96     & 3.96 \\ \hline
	\end{tabular}
	\caption{The scalability experiment results}
	\label{tab:scalability}
	\vspace{-9mm}
\end{table}

==> sections/introduction.tex <==
\section{Introduction}

Large Pretrained Language Models (PLMs) like Bert~\cite{devlin2018bert} 
have been widely adopted in online services related with natural language processing (NLP). 
These PLMs consist of a large number of stacked attention-based layers to learn hierarchical semantic representations for high accuracy.
But the stacked layers significantly increase the computation time and memory footprint for inference.
As results,
large PLMs suffer from high inference latency, 
and they can hardly process the massive user requests simultaneously.

In practice, online NLP services can have strict time Service-Level-Objects (SLOs) to handle stochastic inference workloads. 
A wide range of time-sensitive applications require the low latency for real-time inference.
For example, news sentiment classification for the financial market is expected to be as quick as possible, 
because even 5-10 millionths of a second can determine the profits in the automatic stock trading~\cite{aquilina2022quantifying}.
Information retrieval can have harsh SLOs of 10ms~\cite{yang2020model}, 
so it has to quickly score the document relevance with the user query.
Automatic written language checking needs to give immediate feedbacks while users typing. 
Furthermore, the online workload has two kinds of stochasticities, leading to changes and irregularities. 
One is the stochastic submission pattern of inference request, 
which makes the workload sometimes heavy sometimes light.
The other stochasticity is the various sequence lengths in natural language, 
resulting in irregular computation and storage costs. 
 

\begin{figure}[t]
	 \centering
         \includegraphics[width=\linewidth]{figures/decomposition} \caption{Model Decomposition and Parallelization (MDP): the left is the original teacher model with a large model depth, and the right is the decomposed parallel student models having only two layers while maintaining inference accuracy. }

     \label{fig:comparision}
\end{figure}


% Many studies have been done in the literature to reduce inference latency.
%In the scenario of interactive inference, 
%Because of the sequential layer-by-layer execution of large PLMs,
%the latency is highly related to the model depth (i.e., the number of layers).

The model depth (i.e., the number of layers) linearly increases the computation cost and memory footprint, 
because of the serial computation complexity 
and the storage of different layers.
Consequently,
many studies, 
such as knowledge distillation~\cite{sanh2019distilbert, sun2019patient, jiao2019tinybert}, pruning~\cite{DBLP:conf/rep4nlp/GordonDA20,michel2019sixteen, hou2020dynabert}, 
and adaptive computation~\cite{DBLP:conf/acl/XinTLYL20, DBLP:conf/acl/LiuZWZDJ20,zhou2020bert},
% and class parallelism~\cite{}
have explored how to decrease the model depth for lower latency.
However, to effective learn the hierarchical semantic meanings and maintain the accuracy,
the number of layers that can be decreased is limited.
% existing studies can only decrease a limited layer number 
For instance,
knowledge distillation or pruning cannot guarantee the accuracy 
if the reduced model depth is too small~\cite{jiao2019tinybert,hou2020dynabert},
% compared to the original model 
and adaptive computation requires a large portion of samples to go through all layers 
to achieve high accuracy~\cite{DBLP:conf/acl/XinTLYL20, DBLP:conf/acl/LiuZWZDJ20,zhou2020bert}. 
% and class parallelism~\cite{} cannot prune many layers for one class.
% in the split sub-model for one class. 
%, and it is not suitable for regression and binary classification either.  



Most recently,
the state-of-the-art Cocktail method ~\cite{276950} adopts \emph{bagging ensemble}
to select a subset of small \emph{candidate} models to perform inference in parallel,
the results of which are combined to get the final inference result.
% and combines the results of the small models 
Cocktail reduces inference latency while satisfying the accuracy requirement.
However,
existing ensemble algorithms can only select relatively-fast models 
from the available candidates that have already been trained 
through the aforementioned layer reduction methods,
and the latency of the Cocktail is decided by the largest model in the ensemble.
Therefore,
like previous studies,
Cocktail also suffers from the accuracy-latency dilemma of model inference,
thus being far from satisfactory for time-sensitive scenarios.


%\begin{comment}
Moreover, all previous works have to pay extra time costs for the stochastic workloads. 
Since inference requests arrive in the stochastic order,
previous works usually employ a waiting queue to collect a data batch for the data parallelism on GPU.
Hence, the early arrived samples must endure a longer waiting time.
And if there is unexpected bursty, those works either have to wait for cold started machines
or even cannot handle it at all due to limited resources. 
%The other stochasticity is the various sequence lengths in natural language. 
Additionally, Single Instruction Multiple Data (SIMD) parallelism requires different samples in the same batch to have the regular length, so short sentences need to add extra paddings to form regular data batches.
%\end{comment}

This paper presents Model Decomposition and Parallelization (\sys) to achieve low inference latency and high prediction accuracy for large PLMs.
The key idea of \sys is 
to decompose deep and large PLMs into a group of flat models
(as illustrated in Figure~\ref{fig:comparision}),
which trades more parallel operators for less serial operators to maintain the accuracy.
Different from Cocktail's bagging ensemble
that selects a subset of already-available models having different network archetectures,
model decomposition \emph{generates} a group of new models,
% to replace the original model,
which 
(i) have the same flat network structure to avoid stragglers in parallel model executions,
(ii) is explicitly designed to work together to maintain the accuracy, 
% for parallel inference,
% imbalanced executions between the models
and (iii) is flexible to adjust the model number according to the varying inference workload.
%model decomposition can also benefit resource utilization 
%for lightweight workloads.


To effectively decompose the deep PLMs while keeping high accuracy, 
we propose a novel knowledge-distillation training method,
which gradually transfers the knowledge encoded in the original teacher model
% (referred to as a \emph{teacher})
to a group of parallel flat student models 
% (referred to as \emph{students})
based on boosting ensemble and layer distillation.
%
Specifically,
we train the students \emph{sequentially} % one after another
to correct the final output error 
between the teacher and the group of students, 
so that the output difference can be gradually reduced 
as more students are trained and added to the group. 
%
And each student imitate different layers of the teacher in its intermediate layers to increase diversity and generalization of the ensemble. 
%
Both the depth and the number of the parallel student models are adjustable.
Ideally,
if all student models have only two layers, 
i.e., the theoretical lower bound for non-linear classification,
\sys can minimize the inference latency. %for online inference.
% In addition, 
If necessary, \sys can drop the last-trained students with the minimal accuracy penalty.
% to decrease the student number 
%%%%%%%% ???
% by distilling the sum of previous final representations into its intermediate layer output

% To maintain the accuracy, all students of \sys are sequentially distillate from the original model in training, inspired by the ideas of boosting and stacking ensemble. 
% \sys trains every student to further correct the final representation error between the deep teacher and all previous students so that the output difference can be reduced with more students. 
% And \sys can drop the rear students to decrease the student number with minimal accuracy loss if necessary.
% Although any student has no input dependency on the previous students, \sys virtually stacks every student on the previous ones by distilling the sum of previous final representations into its intermediate layer output.
% Therefore, \sys can reduce the model depth to two attention layers with comparable accuracy, namely the minimal layer number, to realize non-linear classification.

To avoid extra costs for stochastic workloads, \sys has specialized system design to serve the parallel student models to directly infer on individual samples instead of data batches. 
\sys allocates all student models on different GPUs for better parallelization and less redundant storage across different GPUs. 
 To get rid of the waiting queue and extra paddings, it directly dispatches different individual samples to run concurrently instead of large data batches of the same length. 
 And \sys keep tracking the changes of inference workload and reduce the student number for bursty workloads.

We have implemented a prototype of \sys with PyTorch and deployed it on a GPU cluster with 8 GPUs
to conduct comprehensive experiments. 
Evaluation results show that 
\sys outperforms the state-of-the-art baseline by up to 2$\times$
in terms of average and tail inference latency
while achieving the best prediction accuracy in all optimized methods.
Further,
it can get 2.2$\times$ throughputs if it only uses one student model to get competitive prediction accuracy.
If we relax the latency requirement to use the half layers of the teacher, it can even surprisedly outperform the original teacher in accuracy due to the boosting ensemble. 

To summarize, our work make following contributions: 
\begin{enumerate}
	\item We propose the novel \sys to reduce the model depth to the theoretical minimum, namely two layers, to achieve ultra-low latency while maintaining accuracy.
	\item We make specialized system designs to serve parallel student models on the stochastic workloads.
	\item We conduct comprehensive experiments to verify the effectiveness of \sys.
\end{enumerate}




 
\begin{comment}
 %including news sentiment classification~\cite{} for financial market, web search engine~\cite{}, and QA system~\cite{} for customer services. 
  %Therefore, these online inference services usually employ the powerful GPU cluster for short latency. 
 
 % many previous works are attempting to reduce the latency, including knowledge distillation, pruning, quantization, adaptive computation, and bagging ensemble of cheap models. 
 
 There are two reasons for their failures: 
 One reason is that previous works can only decrease a limited layer number in one model to maintain accuracy. The model inference has to conduct serial forward propagation layer by layer, which significantly affects latency. But existing works can hardly further reduce the model depth because multiple stacked attention layers enable effective semantic representation learning. 
 The other reason is that batch inference causes extra latency due to the stochastic and irregular inference workloads. GPU needs batches of samples in the same length for the SIMD parallelism, but inference samples have irregular sentence lengths and arrive independently in the stochastic order. It needs the waiting queue and paddings to form large and regular data batches, resulting in extra time costs for early arrival and short samples.
 
 \begin{itemize}
 	\item No previous works can reduce the model depth to two attention layers without accuracy loss, namely the minimal number to realize non-linear classification. Model inference has to conduct serial forward propagation layer by layer, which significantly affects latency. But it is hard for 2-layer model to achieve comparable accuracy, because attention based models rely on multiple stacked attention layers to effectively learn the semantic representation. For example, due to limited capability, 2-layer student cannot properly imitate the deep teacher model in knowledge distillation. In adaptive computation, some hard samples even still have to go through all layers. Bagging ensemble has to select relatively cheaper models from the trained candidates who all have over two attention layers.

 	\item It brings in tail latency to realize the batch inference on the stochastic workload for better GPU utilization. GPU needs a batch of samples in the same length for the SIMD based data parallelism, but practical inference samples not only have irregular sentence lengths but also arrive independently in the stochastic order. Therefore, inference system usually employ the waiting queue and paddings to form the large and regular data batch. As the results, early arrived samples suffer from longer tail latency, and short samples pays extra costs of time and space for paddings.
 \end{itemize}

 The model layer number is one of the most significant factors determining the inference latency. 
 The attention based models rely on multiple stacked attention layers to effectively learn the semantic representation (\S ~\ref{sec:attention_model}). 
 And model inference has to conduct serial forward propagation layer by layer, while the computations on different channels in the same layer are in parallel. 
 As a result, the model inference latency usually increases linearly with its layer number, which can be further verified by experiments (\S~\ref{sec:layer_exp}).

Various previous works has attempted to reduce the layer number for lower inference latency while maintaining the accuracy. 
Knowledge distillation trains a smaller student model with fewer layers under the guide of original teacher model. 
Adaptive computation~\cite{} can save latency for the simple requests by early exiting from bottom layers. 
Some other works explore how to make use of bagging ensemble of multiple shallow models~\cite{} to achieve the comparable accuracy of the deep model.

But unfortunately, all these works fail to reduce the model to the minimal layer number for ultimately low latency without accuracy loss. In the theory, neural network only needs 2 layers to realize non-linear classification ~\cite{}. 
If the student in the knowledge distillation only has 2 layers, the model capability is too limited to imitate the deep and complex teacher model.
In the adaptive computation, not all samples can ealy exist within the first 2 layers and some hard ones have to go through all layers. 
 Bagging ensemble of different deep models depends on the diversity of model architectures to improve the prediction accuracy, so it has to pick some models with over 2 layers to achieve the target accuracy.
 
 Furthermore, online inference has to bring in tail latency to realize the batch inference for the better utilization of the GPU cluster. Unlike the training has offline data batches in the local storage, online inference has to deal with the samples submitted one by one in the stochastic order. And all inference samples are often irregular due to the different sentence lengths in natural language. In practice, inference system has to use the waiting queue to collect enough samples for the inference in batch mode, which brings in extra tail latency for the early arrived samples. Because GPU needs regular data for the SIMD parallel computation, short sequence samples needs some paddings that costs more time and space for the inference.

the online service of large attention-based model suffers from both high (tail) latency and low cluster utilization in practical inference workloads. It is well known that the large and deep network architecture of attention based models result in high latency in online model service. Although GPU has powerful parallel computation capability~\cite{}, they have to conduct serial forward computations layer by layer. What is more important, online model inference cannot take large data batches of regular samples for granted to employ data parallel for high utilization of the GPU cluster like training. In practices, inference requests of different sequence lengths stochastically arrive one by one instead of data batches of regular samples. Inference on single request or a small data batch cannot fully utilize the massive GPUs in the cluster. And the paddings on the short sequences bring in extra time and space complexities for its inference.
%If employing a waiting queue to form large and regular data batches, the early arrived requests have to endure a high tail latency and shorter sequences have to add extra time and space costs due to paddings. 
%that 

Various previous works have made attempts in either algorithm or system to improve inference efficiency, but they still suffer from the problems of high (tail) latency and low cluster utilization in the practical workload of online model inference:
\begin{itemize}
\item Algorithm level: The algorithmic works make the ideal assumption that inference has data batches of the same sequence length just like training. Pruning~\cite{}, knowledge distillation~\cite{}, and quantization~\cite() mainly focus on the deployment on single edge devices with limited computation and storage capabilities. They optimize some proxy metrics like total FLOPs and parameter number, but they ignore the low utilization of massive parallel devices in the cluster for the practical online inference workloads. Adaptive computation~\cite{} can save some latency for the simple requests by early exiting from bottom layers. But other hard requests still have high tail latency to go through all layers.
\item System level: Existing inference system designs bring in extra idle waiting and interference among requests due to the waiting queue~\cite{},  extra token padding, and irregular model parallelism~\cite{}. In the waiting queue for data batches, arrived requests have to wait until the queue is fulfilled or time exceeds the threshold. 
%Before transferring the data batch from host to GPU, the computation units have to keep waiting. 
And the sequences of different lengths in the same batch have to be padded into the same length at the extra time and space cost. Some works also try to select and ensemble some cheap models in different architectures to reduce the latency. However, the irregular architectures of different models results in the waiting for the slowest model. What is worse, the naive bagging ensemble can hurt the accuracy performance, if the models are too weak.
\end{itemize}

\begin{figure}[t]
	 \centering
     \begin{tabular}{@{}c@{}}
         \includegraphics[width=0.4\textwidth]{figures/data_batch} \\[\abovecaptionskip]
  		 \small (a) Data Batch
     \end{tabular}
     \vspace{\floatsep}
     \begin{tabular}{@{}c@{}}
         \includegraphics[width=0.45\textwidth]{figures/model_batch} \\[\abovecaptionskip]
         \small (a) Model Batch
     \end{tabular}
     \caption{Illustration on the Comparisons between the Data Batch and Model Batch }
     \label{fig:comparision}
\end{figure}

 Motivated by our analysis and observations about how model and data factors influence the latency, we bring up the conception of the model batch by analogy with the data batch as shown in Figure~\ref{fig:comparision}. At its core, \name trade the larger student number for smaller depth to ultimately reduce the layer number and (tail) latency. Inspired by the spirit of boosting and stacking ensemble, \name distillate and refractorize the deep teacher model into a batch of flat student models instead of the single student in previous works. 
Since the batch of flat students has improved the parallelism, it allocates different student models over different GPUs to fully use of the massive GPUs. To eliminate tail latency caused by the waiting queue and paddings, \name dispatches different individual samples to infer concurrently instead of large and regular data batches. 
Specifically \name proposed the novel algorithm of TeleDistill Boosting to sequentially learn a batch of flat student models from the deep teacher model. In the style of boosting ensemble, every student model attempt to further reduce the final representation differences between the deep teacher and all previous students. Based on the idea of stacking, each student model virtually takes the outputs of previous students as the input by distilling the ensemble of all previous student outputs into its intermediate representation. The tele-distillated boosting ensemble of multiply students not only improve the parallelism for inference but also find more rooms to further reduce layer number. 
%All student models have the same computation cost due to the homogenous network architecture. 
By giving up the rear and minor student models in the boosting, \name can also trade the minimum accuracy to process more concurrent inference samples. 

Since the batch of student models improves the parallelism, \name can dispatch different individual inference samples to save the costs of collecting and regularizing the data batch.
\name evenly allocates the batch of student models across different GPUs for balanced workload of massive GPUs. And each GPU can duplicate its student model for the same times to fully utilize the GPU.  \name buffers the inference samples into one of the multi-queue according to their sequence lengths. It only dispatches single sample or a small data batches of the same length to execute the inference. \name schedules different individual samples or data batches to run concurrently on the same GPUs, so that it can achieve better utilization in the pipeline parallelism of different inference samples.
\name also keeps track the intensity of inference workloads and decrease the student number to process more samples if necessary.
\end{comment}



\begin{comment}
(From the system perspective, the inference on multiple flat and regular models are efficient and friendly to GPU parallelism even for only one request. Since one request can fully utilize the GPU, different inference requests are scheduled to different GPUs to avoid long-tail latency caused by mutual interference. From the algorithm perspective, MBBS employs boosting ensemble to achieve multiple flat models equivalent to the original deep model. During the training, every newly added student model contributes more in reducing the  accuracy gap between the original teacher and the ensemble students. If there is a sudden peak in coming workloads, MBBS can elastically and adaptively trade the minimum accuracy loss for larger throughput by giving up the rear and minor students. )


Specifically, we identify that concurency bound is the major system bottleneck for attention-based model inference, which motivates our design that multiple flat students replaces one deep and large teacher. The forward pass through stacked attention layers have to be conducted layer by layer, while the computation of different heads in the same layer is parallel. Inference latency tends to linearly increase with the number of layers other than the amount of heads. Therefore, MBES is designed to consist of multiple flat students in parallel to be friendly to SIMD devices like GPUs. The shallow model depth enable MBES has less serial computation and latency. Furthermore, the structure of  parallel wide models offers enough parallelism to fully utilize SIMD devices even only with one or limited requests.

At algorithm level, we adopt adaboosting ensemble to maintain accuracy with much less attention layers. Original teacher model needs dozens of stacked attention layers to extract complex semantic features and patterns and achieve high accuracy. Although the previous model compression works have attempted to reduce the layer number, MBES can find even more potential  room by adaboosting multiple shallower and weaker students. The adaboost sequentially trains those multiple flat student models and each newly added student tries its best to correct the residual errors of all previous models. To improve generalization and training speed, we further take advantage of the guide from the large teacher model by weight transfer and knowledge distillation. In the case that the coming workloads exceed the whole system capability, MBES can adaptively give up the rear student models who has minor accuracy contributions to handle more requests with the minimum accuracy loss. 


In summary, we makes three key contributions in the proposed \name as follows:
\begin{enumerate}
	\item Through analysis and observations we identify the gap between high (tail) latency and low utilization in the practical inference workloads, and we further brings up the conception of model batch for the stochastic requests of different lengths.
	\item \name propose a novel co-design of algorithm and system to realize the model batch. It brings in the new teleDistill Boosting algorithm to trade larger width for smaller depth. It also employs new resource management and task scheduling free of waiting queue and extra token paddings.
	\item We make the full implementation and conduct comprehensive experiments to verify the effectiveness to fill the gap and significantly improve the inference efficiency without much accuracy loss.
\end{enumerate}
\end{comment}

% Ideally, the online inference system should realize two goals for the practical inference workload as follows:
% \begin{itemize}
% 	\item \textbf{Low (tail) latency}: It should respond to each sample as soon as possible to enable time-sensitive applications. Different inference samples should avoid interfere with each other to cause tail latency for some samples. 
% 	\item \textbf{High accuracy}: The inference system is not expected to trade much accuracy for inference latency, since accuracy is important for many applications.
% 	%\item High utilization: It should fully utilize the massive and powerful GPUs in the cluster to offer accurate and efficient online inference service. 
% 	%\item High Throughput: It should be also able to deal with the intensive hurricane workload~\cite{} for some special occasions.
% \end{itemize}


% Although many previous works have optimized the latency, none can achieve the ultra-low (tail) latency without accuracy loss. Inference latency increases linearly with the model depth due to the serial computation layer by layer, but multiple stacked attention layers enable the effective semantic representation learning. 
% Therefore, previous works can only decrease limited layer number in one model to maintain the accuracy. Knowledge distillation~\cite{} or layer pruning~\cite{} cannot achieve comparable accuracy if the model depth is too small in one model. In adaptive computation~\cite{}, some hard samples still have to go through all layers. Bagging ensemble~\cite{} can only select relatively faster models from the candidates readily trained in above mentioned methods, who all have multiple stacked attention layers. Class parallelism cannot prune many layers in the split sub model for one class, and it is not suitable for regression and binary classification either.  
%Additionally, waiting queue~\cite{} and paddings~\cite{} causes extra latency for early arrived samples and the short ones respectively to form a large and regular inference batch.

%the TeleDistill Boosting algorithm that refactorizes the deep attention-based model by distilling it into a batch of flat student models other than only one.
%At its core, it trades more significant model numbers for less depth under the accuracy constraint.

==> sections/introduction_backup.tex <==
\section{Introduction}

Nowadays extremly large attention-based models inspired by the transformer structure are dominating the field of Nature Language Processing(NLP). Popular online services like information retrieval, financial sentiment classification and  product recommendation have widely adopted attention-based models like BERT and its variants, leading to one of the biggest leap in the past decades. The attention-based models have the complex and stacked attention mechanism and an unprecedentedly large number of parameters. After pretrained on a large corpus, they have achieved significant accuracy advantages over previous models(e.g. CNN and RNN) and even outperformed human beings in challenging sentence classification tasks.  

But unfortunately, inference system hosting large attention-based models suffer from low efficiency when dealing with live and stochastical requests in practical workloads. Firstly, stacked complex attention layers and numerous parameters result in high inference latency, which significantly influences user experiences and even violates service level objectives (SLOs). More importantly, inference system needs to handle dynamical and various workloads in practice, which keep changing over time and have large variances among different applications. Different from the training that all data samples are ready to form mini-batches, real requests of online service arrive in a stochastical order. On the one hand, there is no guarantee that a batch of samples will arrive simultaneously in the inference phase to trivially realize data parallel. Some applications even urgently require fast inference on single live data, which only have one atomic data item every time. Taking the learning based automatic stock trading as one example,  it is very sensitive to latency and only makes inference on the latest signals at every step. However, SIMD devices like GPU with high parallel capability can be concurrency bounded and underutilized to speed up single or limited inference samples in such situations. On the other hand, there can be massive requests suddenly crowding into the online service on some special occasions. For example, breaking news can suddenly attract numerous users to search related stories and backgrounds. In such a case, inference system can be overloaded with limited hardware resources, and overwhelming workloads are leading to high latency that violates SLOs and damages user experiences.

There has been various efforts related to improve attention-based model inference efficiency in differnt levels from top to 
\begin{itemize}
\item Algorithm Level:  Although machine learning community has developed many methods (e.g. pruning, knowledge distillation, quantization and adaptive computing), these works make the ideal assumption that inference is in batch mode just like training. Algorithm-level works only reduce some proxy metrics (e.g. Flops and memory size) instead of directly improving system bottlenecks (e.g. concurrency, memory  and computation bounds). These works mainly focus on the deployment in edge devices with limited computation and storage capabilities, they suffer from inferior inference performance in the data center hosting online services because of not explicitly considering the characters of the system and devices  to exploit high parallelism capability . Additionally, these algorithm-level works usually trade some accuracy for inference efficiency.
\item System Level: Existing inference systems have made attempts on the waiting queue,  proper model selection and class parallelism, but they still bring in extra idle waiting time. In the waiting queue for dynamic batches, the earliest request has to wait until the queue is fulfilled by a batch of requests or it reaches the time threshold.  The model variants satisfying SLOs, selected from a given set of fixed model candidates, usually have irregular network architectures, resulting in idle waiting for the straggler.  Futhermore, due to the correlation of given model candidates, ensemble of selected models can hardly fulfill the large accuracy gap between a large attention-based model and the selected small ones, especially if the SLO is small. SensAI introduces the class parallelism by decoupling a mutli-class CNN into several pruned networks responsible for predicting different classes. However, class parallelism is not suitable for  popular regression(e.g. ranking) and binary classification(e.g. Sentiment or relevant classification) tasks in NLP. 
\item Hardware Level: Application-specific Integrated Circuit(ASIC) devices (e.g. DianNao and TPU) have been developed to speed up both training and inference, but they also follow the ideal batch assumption. What is worse,  it costs a long time and large R\&D expenses to deliver final ASIC production. They are not flexible for new operators or widely available in common situations. 
\end{itemize}

In short words, despite all previous workers at different levels, the large attention-based mode still suffers a lot when making inference on live and stochastical data in the production environment. Ideally, the large attention-based model inference system should realize three goals as follows:
\begin{enumerate}
	\item Low (tail) latency: The inference system should respond to each request in short latency and different requests should not interfere with each other to bring in long-tailed latency. Hence, the inference system can even enable inference on live data or limited requests, satisfy applications' SLOs, and improve user experiences for all requests.
	\item Maintaining accuracy: The inference system is not expected to trade accuracy for inference efficiency, since accuracy performance is critical for many applications(e.g. Search for proper information and stock trading).
	\item Flexibility and Elasticity: The inference system is supposed to support any practical workload no matter it has only single live data or crowded requests. For the single or limited requests, inference system is still preferred to fexibily utilize SIMD devices to speed up them properly. If running into overwhelming requests, it is better to be elastic to achive larger throughput even if no extra resources can be availale in a short time.
\end{enumerate}

Therefore, to realize all three design goals, we propose the Model Batch of Ensemble Students(MBES) framework, a novel co-design at both algorithm and system levels. At its core, MBES learns a batch of shallow and regular student models from one deep and complex teacher model in the style of adaboosting ensemble, which is explicitly designed for GPU's high parallelism capability.  From the system perspective, the inference on multiple flat and regular models are efficient and friendly to GPU parallelism even for only one request. Since one request can fully utilize the GPU, different inference requests are scheduled to different GPUs to avoid long-tail latency caused by mutual interference. From the algorithm perspective, MBES employs boosting ensemble to achieve multiple flat models equivalent to the original deep model. During the training, every newly added student model contributes more in reducing the  accuracy gap between the original teacher and the ensemble students. If there is a sudden peak in coming workloads, MBES can elastically and adaptively trade the minimum accuracy loss for larger throughput by giving up computation of rear and minor students. 

Specifically, we identify that concurency bound is the major system bottleneck for attention-based model inference, which motivates our design that multiple flat students replaces one deep and large teacher. The forward pass through stacked attention layers have to be conducted layer by layer, while the computation of different heads in the same layer is parallel. Inference latency tends to linearly increase with the number of layers other than the amount of heads. Therefore, MBES is designed to consist of multiple flat students in parallel to be friendly to SIMD devices like GPUs.  The shallow model depth enable MBES has less serial computation and latency. Furthermore, the structure of  parallel wide models offers enough parallelism to fully utilize SIMD devices even only with one or limited requests.

At algorithm level, we adopt adaboosting ensemble to maintain accuracy with much less attention layers. Original teacher model needs dozens of stacked attention layers to extract complex semantic features and patterns and achieve high accuracy. Although the previous model compression works have attempted to reduce the layer number, MBES can find even more potential  room by adaboosting multiple shallower and weaker students. The adaboost sequentially trains those multiple flat student models and each newly added student tries its best to correct the residual errors of all previous models. To improve generalization and training speed, we further take advantage of the guide from the large teacher model by weight transfer and knowledge distillation. In the case that the coming workloads exceed the whole system capability, MBES can adaptively give up the rear student models who has minor accuracy contributions to handle more requests with the minimum accuracy loss. 

In summary, our MBES framework makes key contributions as follows:
\begin{enumerate}
	\item We compress the large attention-based model into the ensemble of flat students instead of one student, which enable reducing more layer numbers for short latency without accuracy loss.
	\item The multiple flat student models also make up a Model Batch so that even the inference on single request can fully utilize GPU to be accelebrated. It also realizes flexible and direct request dispatching without the waiting queue and any interfere between requests. 
	\item MBES offers an elastic way to serve overwhelming workload with limited hardware resources by trading minimum accuracy for larger throughput.
\end{enumerate}

==> sections/preliminary.tex <==
\section{Preliminary and Background}

==> sections/relatedwork_backup.tex <==
\section{Related Work}

\label{sec:existing_work}
There are three limitations of existing works 
to realize low-latency and high-throughput inference for LLMs in processing online workloads, as discussed in the rest of this section.
\subsubsection{Deep Network Architecture}

Existing works try to reduce overall computations and model size but do not directly optimize the amount of serial computations.
Knowledge distillation~\cite{sanh2019distilbert, sun2019patient, jiao2019tinybert} trains a single student model with guidance from a large and deep teacher model. 
The single student can have smaller width in each layer but still requires a considerable model depth to maintain good accuracy. 
For example, 6-layer DistillBERT can maintain 96.3\% overall score of the teacher, but the 3-layer PKD-BERT can only get 88.5\% (\S~\ref{sec:accuracy}). 
Pruning removes redundant weights, neurons, or even attention heads of well-trained LLMs and then fine-tunes the remained parts for better generalization,
but it usually cannot remove an entire layer. 
Like knowledge distillation, it has a limited ability to reduce the model depth while maintaining accuracy~\cite{hou2020dynabert}. 
Adaptive computation~\cite{DBLP:conf/acl/XinTLYL20, DBLP:conf/acl/LiuZWZDJ20,zhou2020bert} allows early exit before executing the last few layers for "easy" samples, but "difficult" samples still need to go through all layers, resulting in long-tail latency.
he mixture-of-experts structure~\cite{DBLP:conf/iclr/ShazeerMMDLHD17,DBLP:conf/naacl/ZuoZLHZC22} only activates one or two experts in each layer,
 so it can keep constant inference cost no matter how wide the model is. However, it cannot decrease the model depth either.

SenseAI~\cite{wang2021sensai} divides the multi-class model into several pruned binary sub-networks. 
Each sub-network still has a large model depth and irregular pruned architecture and cannot be used in regression (e.g., ranking) and binary classification (e.g., sentiment or similarity classification) tasks. 

Clipper~\cite{DBLP:conf/nsdi/CrankshawWZFGS17} and Cocktail~\cite{276950} adopt \emph{bagging ensemble} to select a subset of small candidate models to execute in parallel for lower latency and combine all results by averaging or voting for high accuracy.
However, all the available candidate models have already been trained by the aforementioned methods without knowing each other. 
These candidate models inherently have a considerable number of layers, and the slowest model in the ensemble decides their inference latency. 
 
